Clustered Sampling: Low-Variance and Improved Representativity for Clients Selection in Federated Learning

This work addresses the problem of optimizing communications between server and clients in federated learning (FL). Current sampling approaches in FL are either biased, or non optimal in terms of server-clients communications and training stability. To overcome this issue, we introduce \textit{clustered sampling} for clients selection. We prove that clustered sampling leads to better clients representatitivity and to reduced variance of the clients stochastic aggregation weights in FL. Compatibly with our theory, we provide two different clustering approaches enabling clients aggregation based on 1) sample size, and 2) models similarity. Through a series of experiments in non-iid and unbalanced scenarios, we demonstrate that model aggregation through clustered sampling consistently leads to better training convergence and variability when compared to standard sampling approaches. Our approach does not require any additional operation on the clients side, and can be seamlessly integrated in standard FL implementations. Finally, clustered sampling is compatible with existing methods and technologies for privacy enhancement, and for communication reduction through model compression.

==> tex/applications.tex <==
\subsection{Improvements provided by clustered sampling}

FedProx sampling and clustered sampling both satisfies Assumption \ref{ass:sampling} and have the same theoretical properties at convergence, Theorem \ref{theo:convergence_clustered}. However, when considering the stochastic weight of a client $\omega_i(t)$ at a given iteration, clustered sampling has better properties than FedProx sampling scheme. To differentiate between FedProx sampling and clustered sampling, we respectively define $S_{FP}$ and $S_C$ as their subset of sampled clients.

Both sampling schemes respect Assumption \ref{ass:sampling}. Hence, for the two sampling schemes, the expected aggregation equals to the one when considering all the clients leading to:
\begin{equation}
	\EE{S_{FP}}{\omega_i(S_{FP})}= p_i
	\text{ and }
	\EE{S_C}{\omega_i(S_C)} = p_i . 
\end{equation}

However, every clients with clustered sampling schemes has a smaller weight variance for any set of $m$ distributions $\{S_k\}_{k=1}^m$ than with FedProx sampling scheme. We can first rewrite the weight $\omega_i(S) = \frac{1}{m}\sum_{k=1}^{m}\{ l_k(t) = i\}$. For FedProx, $m$ clients are sampled independently with the same distribution $S_0$. As such, the variance of a client's weight is the sum of $m$ identical Bernoulli distribution with probability $p_i$ giving the following variance:
\begin{align}
	\VARR{S_{FP}}{\omega_i(S_{FP})}
	&= \frac{1}{m^2}m \VARR{S_0}{\{l_1 = i\}}\\
	&= \frac{1}{m^2}m p_i(1-p_i) .
\end{align}
For clustered sampling, the distribution is specific to the index $k$. However, clients are still sampled independently. As such, the variance of a client;'s wight is the sum of $m$ different and independent Bernoulli distribution each with probability $r_{k,i}$ which gives:
\begin{align}
\VARR{S_{C}}{\omega_i(S_C)}
&= \frac{1}{m^2} \sum_{k=1}^{m} \VARR{S_k}{\{l_k = i\}}\\
&= \frac{1}{m^2} \sum_{k=1}^{m} r_{k,i}(1-r_{k,i}) .
\end{align}

By using the Cauchy Schwartz inequality, one can prove that 
\begin{equation}
	\VARR{S_{FP}}{\omega_i(S_{FP})}
	\ge \VARR{S_{C}}{\omega_i(S_C)}.
\end{equation}
The exact derivation can be found in Appendix \ref{app:stat_measure_clust_2}.

Another interesting property is the probability of a client of being sampled, i.e. $\{i\in S_t\}$, in any of the two sampling schemes. This criteria is different from the expected weight of a client. Indeed, if a client has an higher probability of being sampled it means that at every iteration, on the sampled specific to the distribution of the client, the global model forgets less . For this criteria, clustered sampling also outperforms FedProx sampling scheme. Using the fact that the clients are sampled identically and independently for every position $k$, FedProx gives:
\begin{align}
p(i \in S_{FP})
&= 1 - p(i \notin S_{FP})\\
&= 1 - p(\{i \notin S_0\})^m\\
&= 1 - (1-p_i)^m .
\end{align}
Similarly, clustered sampling gives:
\begin{align}
p(i \in S_C)
&= 1 - \prod_{k=1}^m p(\{i \notin S_k\})\\
&= 1 - \prod_{k=1}^m (1- r_{k,i})
\end{align} 
Clustered sampling follows Assumption \ref{ass:sampling}. Hence, by using equation \ref{eq:total_probability} and the AM-GM inequality, we get:
\begin{equation}
p(\{i \in S_{FP}\}) 
\le
p(\{i \in S_C\}).
\end{equation}
The exact derivation can be found in Appendix \ref{app:stat_measure_clust_2}.

%\begin{figure*}
%	\centering
%	\begin{tabular}{ |l||l|l|l|  }
%		\hline
%		& A - FedProx & B - Clustered sampling II & Comparison\\
%		\hline
%		$\EE{S}{w_i(S)}$ &$p_i$ & $p_i$  & $A = B$ \\ \hline
%		
%		$\VARR{S}{w_i(S)} $ 
%		& $\frac{1}{m^2} m p_i (1- p_i)$ 
%		& $\frac{1}{m^2}\sum_{j=1}^{m} r_{ji} (1- r_{ji})$
%		&$A\ge B$\\ \hline
%		
%		$p(\{i \in S\})$ 
%		& $1 - (1- p_i)^m$ 
%		& $1 - \prod_{j=1}^m (1- r_{ji})$
%		&  $A\le B$\\
%		
%		\hline
%	\end{tabular}
%	\caption{Summary table of the different statistical measures for FedProx and Clustered Sampling II.}
%	\label{tab:clustered_2_stats}
%\end{figure*}

In conclusion clustered is a sampling scheme reducing the weight of variance of every client as well as increasing the probability of every client of being sampled. These results are very important as in FL, data is often non-iid and can be client specific. Therefore, increasing the probability of every client of being samples ensure that the client with unique distributions are more likely of being sampled and therefore the global model at a given iteration is more likely to get a data support closer to the one of all the clients.

\subsection{Creating the distribution}\label{sec:basic_clustered}


We have shown in Section \ref{sec:clustered_sampling} that as long as clustered sampling is unbiased, Assumption \ref{ass:sampling}, its convergence guarantees toward a local minimum are identical to the ones for FedProx's sampling and in addition at every iteration the stochastic aggregation is further improved with clustered sampling. 

While every clustered sampling satisfying Assumption \ref{ass:sampling} is an improvement, we are interested here in creating clusters minimizing the total client's weight variance. Hence, we define $F(\{r_{k,i}\}) = \sum_{i=1}^{n}\VARR{S_C}{\omega_i(S_C)} = \sum_{i=1}^{n}\frac{1}{m^2} \sum_{k=1}^{m} r_{k,i}(1-r_{k,i})$. Given that we want to find distribution for a clustered sampling following Assumption \ref{ass:sampling}, equation \ref{eq:sum_proba} and \ref{eq:total_probability} are constraints for our optimization problem. Thus, we can rewrite the loss function as $F(\{r_{k,i}\}) = \frac{1}{m}- \frac{1}{m^2}\sum_{i=1}^{n} \sum_{k=1}^{m} r_{k, i}^2$.
Thus, by rewriting the loss function we try to optimize the following optimization problem:
\begin{align}
	&\min_{\{r_{k,i}\}} \frac{1}{m}- \frac{1}{m^2}\sum_{i=1}^{n} \sum_{k=1}^{m} r_{k, i}^2\\
	&\text{subject to } \nonumber\\
	&\forall k \in\{1, ..., m\},\ \sum_{i=1}^{n}r_{k, i} = 1 \text{ with } r_{k, i} \ge 0\\
	&\forall i \in \{1, ..., n\},\ \sum_{k=1}^{m} r_{k,i} = m p_i
\end{align}
This optimization problem has a minimum has a finite global minimum. However, as this optimization problem can be rewritten as a quadratic optimization with a negative semi-definite matrix and convex constraints, solving this optimization problem is NP-Hard. Here we are trying to optimize the sum of each client's variance. When considering minimizing the variance of only one client, we get the following optimization problem:
\begin{align}
&\min_{\{r_{k,i}\}} \frac{p_i}{m}- \frac{1}{m^2}\sum_{k=1}^{m} r_{k, i}^2\\
&\text{s. t.} \sum_{k=1}^{m} r_{k,i} = m p_i \text{ with } r_{k, i} \ge 0
\end{align}
This optimization problem can still be rewritten as a quadratic problem with negative eigen values and as such is NP-Hard. However, we can show that the global minimum is attained when setting as many $r_{ki}$ as possible to 1 and give $m p_i - \floor*{m p_i}$ to a remaining client. As such the global minimum is $\floor*{m p_i} + (mp_i - \floor*{m p_i})^2 $ and can be achieved with many combinations. Therefore, we propose Algorithm \ref{alg:clustered_basic} to create the different clients' distributions based on the ratio of samples $p_i$ owned by each client. In this algorithm, every client can be sampled up to $\floor*{m p_i} + 2$ times.

\begin{algorithm}[tb]
	\caption{Clustering clients}
	\label{alg:clustered_basic}
	\begin{algorithmic}
		\STATE {\bfseries Input:} $\{p_i\}$ ratio of samples owned by each client
		\STATE Order the clients by descending importance of $p_i$.
		
		\STATE $k \leftarrow 1$ where $k$ is the distribution index.
		
		\STATE $\forall k,\ q_k \leftarrow 0$; sum of the probabilities in cluster $k$
		
		\STATE $\forall k,\ i,\ r_{k, i} \leftarrow 0$; 

		\FOR{each client $i=1$ {\bfseries to} $n$}
		
			\REPEAT
			
				\STATE $r_{k,i} = \min\{ m p_i, 1 - q_k\}$; client $i$ can be sampled in $S_k$ with probability $r_{k,i}$
				
				\STATE $p_i \leftarrow p_i - \frac{1}{m}r_{k,i}$
				\STATE $q_k \leftarrow q_k + r_{k,i}$
				
				\IF{$q_k = 1$}
					\STATE $k \leftarrow k + 1$
				\ENDIF
		
			\UNTIL{$p_i=0$}

		\ENDFOR
	\end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:clustered_basic}, when summing the probabilities of client $i$ over all the distributions, we get $\sum_{k=1}^{m}r_{k, i} = m p_i$. Similarly, when summing all the probabilities within a distribution, we get $\sum_{i=1}^{n}r_{k, i} = 1$. As such, Algorithm \ref{alg:clustered_basic} satisfies equation \ref{eq:sum_proba} and \ref{eq:total_probability} are respected and therefore Assumption \ref{ass:sampling} holds. Thus the $m$ distributions given by Algorithm \ref{alg:clustered_basic} gives a sampling scheme satisfying Theorem \ref{theo:convergence_clustered}.



\begin{figure}\label{fig:mnist_non_iid}
	\includegraphics[width=\linewidth]{./pics/plot_fig_basic_MNIST.pdf}
	\caption{Comparison between the sampling scheme proposed by FedProx and a perfect sampling scheme sampling 10 clients each with a different digit.}
\end{figure}



\subsection{Further improving client selection}\label{sec:clustered_improved}

\input{./tex/figure_gradients.tex}


As shown in Section \ref{sec:clustered_sampling}, sampling clients with clustered sampling can only provide a smaller or equal variance for each client's stochastic aggregation weight and as such can only improve the convergence speed and decrease the learning process variance.

What we propose now is to improve clustered sampling obtained with Algorithm \ref{alg:clustered_basic}. In Section \ref{sec:basic_clustered}, the proposed algorithm can be seen as considering a unique distribution per client. Indeed, we minimize the variance of the stochastic weight of every client. However, in most federated learning applications, the data distribution is non-iid and client specific. Nonetheless, one can expect some clients to have a similar distribution to some other clients and a completely different from the remaining clients.

Should the server be able to cluster the clients by similarity, what we would be interested in is for an improved clustered sampling to put similar clients together. Another way of formulating is that we would like the server to run Algorithm \ref{alg:clustered_basic} on clusters of similar clients instead of independent client. In turn, it would help minimize the stochastic weight of a type of distribution within the clients' sample distribution. 

Clustering clients by similarity remains possible. \cite{CFL} first proposed a framework clustering clients at convergence based on their similarity. In Figure \ref{fig:schematic_sim} is illustrated how this method would work when considering all the clients. $\theta^t$ is the current global model and $\theta_i^t$ is the updated local model of client $i$ while trying to converge to the local optimum $\theta_i^*$. In practice, clustering clients in function of their updates works quite well as shown in \cite{CFL}. 

This similarity detection process is convenient and its efficiency is shown when considering all the clients in \cite{CFL}. In this work, we propose extending this process to clients' sampling. When considering all the clients, all the local updates $\theta_i^t$ have the same initial point, the current global model $\theta^t$ while when sampling clients the most recent local update for every client is not obtained at the same iteration. In function of the initial model of the learning process, the local work is going to converge to a different local optimum. We consider that between two server iterations, the federated learning process seen from the server point of view is smooth enough that we can consider that the global model are close in comparison of the updated local models $\theta_i^t$ and that similarly, the local optima remains close enough from iteration to the next. We show in practice that even with very non-iid data and non convex assuming these two points give us the expected results. 

As such, when comparing the similarity of clients at a given iteration, we 

In Figure \ref{fig:schematic_sim}, we show a similar schematic to when considering all the clients where for iteration $t$ and $t+1$, the same local optima for the four clients are conserved.

Comparing the updates of the sampled different clients at a given iteration can be done similarly as when considering all the clients at a given iteration. However how to compare the clients sampled at a given iteration with the clients at the next iteration? For each client, we propose comparing the difference between the latest updated local model with its sent global model. We consider that there is a neighborhood such that all the clients are always converging to the same local optimum and the global models' parameters' changes are small enough such that the work obtained at with a given iteration global model would be similar to the one obtained at the next iteration global model.






 


We start clustering from the first iteration. We consider that only starting of $T_0$, the server global model is in the neighborhood allowing the similarity measures to be accurate. For the server iterations $t < T_0$, the clustering is inefficient and federated learning with clustered sampling II has a same behavior as with FedProx sampling scheme. For $t\ge T_0$, the data distribution of the sampled clients is closer to the one of all the clients that for FedProx. As such, there is less forgetting from one iteration to the next and thus faster convergence. In the case where $T_0$ is at infinity is not a problem because as seen in Figure \ref{tab:clustered_2_stats}, the variance of clustered sampling II cannot be bigger than the one of FedProx and the probability a client is sampled cannot be lower than the one of FedProx. Also, Theorem \ref{theo:convergence_clustered} shows that federated learning with clustered sampling II has the same asymptotic behavior as with FedProx sampling, Theorem \ref{theo:convergence_FP}. In practice, we show in the experiments that clustered sampling works on every experimental scenarios with a training speedup for non-iid data and identical training speed for iid data.




In addition, the clients are considered as having non-iid distributions. As such, clustered sampling tries to sample clients at every iteration such that the data distribution of the sampled clients is as close as possible to the one of all the clients.




Based on this fact, we propose a clustering method based on clients' similarity. Clients' similarity has been studied and used for clustering \cite{CFL}[XXX] and for attackers' detection for Byzantine attacks, label flipping, or data poisoning[XXXX]. The underlying method is to compare a clients' local update to its sent model:
\begin{equation}
	\theta_i^{t+1} - \theta^t
	= - \eta \sum_{e=0}^{E-1} g(\theta_i^{t,e}, \xi_e),
\end{equation}
where $\eta$ is the learning rate and $g(\cdot,\cdot)$ is the gradient function estimated on $\theta_i^{t,e}$ the local model obtain after $e$ SGD and on batch of samples $\xi_e$. If $E$ goes to infinity, then $\theta_i^{t+1}$ goes to the local optimum of the loss function of client $i$, i.e. $\theta_i^*$. However, with a fix $E$, the server can only compare this difference in local and global model between each client to infer similarity. No formal proof has been provided so far on how to use this quantity. However, it enables efficient clustering improving global model performance at the end of the training \cite{CFL} AND OTHERS. However, similarity has been investigated when considering all the clients and has never been used at the best of our knowledge for client sampling. 




Our clustering sampling is dynamical. While the sampling distribution is identical at every iteration, the different clusters should be found at every iteration. We propose Algorithm \ref{alg:sampling_clus_2} to obtain the distribution distribution of clients' cluster at every iteration. The participating clients at a given iteration are obtained as follow:
\begin{enumerate}
	\item Get the latest work representation of all the clients
	\item Get the similarity matrix of all the clients' work using Walds' Theorem XXXX.
	\item Create the $m$ distributions of clients using Algorithm \ref{alg:sampling_clus_2}. 
	\item Sample $m$ clients.
	\item Replace the latest work of the $m$ sampled clients.
\end{enumerate}

It is important to notice that at the beginning of the sampling, some clients do not have a representation. As such, we consider that their latest work is the current global model. Therefore for the clients that have never been sampled, there latest work representation is a 0 vector.

%With this proposed method, at every iteration, the weight of each client in the expected value is still $p_i$ (by definition). However, we want to know the difference in variance between our proposal and FedProx. We also want to know the probability a given client is sampled.


%With the current sampling scheme with replacement, some clients can be sampled many times at a given iteration while not being sampled anytime at the next. In expected value, the sampling is defined such that it follows equation XXX. However, the variance of the proposed sampling is such that the convergence speed is lowered. 

%Measure the similarity between the different clients contribution has been studied for clustering XXX as well as for detection of attacks aiming at changing the converging model(Byzantine attacks, label flipping, data poisoning, ...). These works consider a server sampling all the clients at every iteration and, at the best of our knowledge, no work has been currently conducted to measure the similarity between the different clients when the server sample clients.


%\begin{algorithm}[tb]
%	\caption{Clustering clients for Clustered sampling II}
%	\label{alg:sampling_clus_2}
%	\begin{algorithmic}
%		
%		\STATE {\bfseries Input:} $G_i$ representative gradient for each worker, \textit{clustering theorem} (e.g. Ward's theorem), $s$ similarity function 
%		\STATE Compute similarity matrix $M$ with $m_{ij} = s(G_i, G_j)$, the similarity between client $i$ and $j$.
%		\STATE Cluster clients in $m$ clusters, $S_1,...,S_m$,  with \textit{clustering theorem} from $M$. $r_{ki}$ is the probability of client $i$ to be sampled in $S_k$. 
%		\STATE $\forall k\in\{1,...,m\},\ q_k  \leftarrow \sum_{i = 1}^n r_{ki} $ 
%		\STATE $R\leftarrow \emptyset$, set of removed clients and their associated probabilities
%		
%		\FOR{cluster $k=1$ {\bfseries to} $m$ such that $q_k > \frac{1}{m}$} 
%		
%		\REPEAT
%		\STATE Sample a random client $i$ in $S_k$
%		\STATE $u_i \leftarrow \min\{p_k -\frac{1}{m}, p_i \}$
%		\STATE Client $i$ can be sampled in $R$ according to $u_i$
%		\STATE $r_{ki} \leftarrow r_{ki} - u_i$ and $p_k \leftarrow  p_k - u_i$
%		\UNTIL{$p_k = \frac{1}{m}$}
%		
%		\ENDFOR
%		
%		\FOR{cluster $k=1$ {\bfseries to} $m$ such that $p_k < \frac{1}{m}$}  
%		
%		\REPEAT
%		\STATE Sample the first client $i$ in $R$ such that $u_i \neq 0$
%		\STATE $v_{i} \leftarrow \min\{\frac{1}{m}-p_k, u_i \}$
%		\STATE Client $i$ can be sampled in $S_k$ according to $v_i$
%		\STATE $u_i \leftarrow u_i - v_i$ and $p_k \leftarrow  p_k + v_i$
%		\UNTIL{$p_k = \frac{1}{m}$}
%		
%		\ENDFOR
%		
%		\STATE {\bfseries Output:} $S_1,..., S_m$, clusters of clients with sampling probability $r_{ki}$.
%	\end{algorithmic}
%\end{algorithm}

\begin{algorithm}[tb]
	\caption{Clustering clients for Clustered sampling II}
	\label{alg:sampling_clus_2}
	\begin{algorithmic}
		
		\STATE {\bfseries Input:} $G_i$ representative gradient for each worker, \textit{clustering theorem} (e.g. Ward's theorem), $s$ similarity function 
		\STATE Compute similarity matrix $M$ with $m_{ij} = s(G_i, G_j)$, the similarity between client $i$ and $j$.
		\STATE Cluster clients in $m$ clusters, $S_1,...,S_m$,  with \textit{clustering theorem} from $M$. 
		\STATE $r_{ki}\leftarrow m p_i$, for client $i$ if in $S_k$. Otherwise $r_{ki}\leftarrow 0$
		\STATE $\forall k\in\{1,...,m\},\ q_k  \leftarrow \sum_{i = 1}^n r_{ki} $ 
%		\STATE $R\leftarrow \emptyset$, set of removed clients and their associated probabilities

		\STATE Order the clusters by decreasing $q_k$
		
		\STATE $ l \leftarrow m$
		
		\FOR{cluster $k=1$ {\bfseries to} $m$} 
		
		\REPEAT
		\STATE Sample a random client $i$ in $S_k$
		\STATE $u_i \leftarrow \min\{q_k - 1, r_{ki}, 1 - q_l\}$
		\STATE Client $i$ can be sampled in $S_l$ according to $u_i$
		\STATE $r_{ki} \leftarrow r_{ki} - u_i$ and $q_k \leftarrow  q_k - u_i$
		\STATE $r_{li} \leftarrow r_{li} + u_i$ and $q_l \leftarrow  q_l + u_i$
		\IF{$q_l = 1$}
		\STATE $l \leftarrow l - 1$
		\ENDIF
		\UNTIL{$q_k = 1$}
		
		\ENDFOR
		

		
		\STATE {\bfseries Output:} $S_1,..., S_m$, clusters of clients with sampling probability $r_{ki}$.
	\end{algorithmic}
\end{algorithm}








==> tex/figure_gradients.tex <==

% \begin{figure}
% \begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

% %Global models
% \node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
% \node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-7/4/2, -7/2/4){} ;

% %Connect the globsl models
% \draw [line width=1pt, ->] (A)-- (B);
% %	\draw [line width=1pt, ->] (B)-- (C);
% %	
% %Local optima and local update
% \node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-3.5){} ;
% \node[fill, draw, circle,label=left: $\theta_1^t$, minimum size = 3pt, inner sep =0] (F) at (-0.5/2,-3.5/2){} ;

% \node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
% \node[fill, draw, circle,label=right: $\theta_2^t$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

% \node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3.5,0){} ;
% \node[fill, draw, circle,label=above: $\theta_3^t$, minimum size = 3pt, inner sep =0] (J) at (-3.5/2,-0/2){} ;

% \node[fill, draw, circle,label=left: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3, 0.5){} ;
% \node[fill, draw, circle,label=below: $\theta_4^t$, minimum size = 3pt, inner sep =0] (L) at (-3/2,0.25){} ;

% %Connect the updates
% \draw [line width=0.5pt, ->] (A)-- (F);
% \draw [line width=0.5pt, dashed] (F)-- (E);

% \draw [line width=0.5pt, ->] (A)-- (H);
% \draw [line width=0.5pt, dashed] (H)-- (G);

% \draw [line width=0.5pt, ->] (A)-- (J);
% \draw [line width=0.5pt, dashed] (J)-- (I);

% \draw [line width=0.5pt, ->] (A)-- (L);
% \draw [line width=0.5pt, dashed] (L)-- (K);


% %\end{scriptsize}
% \end{tikzpicture}
% %	\hspace{1cm}
% \begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

% %Global models
% \node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
% \node[fill, draw, circle,label=right: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-3/2/2, -3/2/2){} ;
% \node[fill, draw, circle,label=below: $\theta^{t+2}$, minimum size = 3pt, inner sep =0] (C) at (-1.6, -1.15){} ;

% %Connect the globsl models
% \draw [line width=1pt, ->] (A)-- (B);
% \draw [line width=1pt, ->] (B)-- (C);
% %	
% %Local optima and local update
% %Local optima and local update
% \node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-3.5){} ;
% \node[fill, draw, circle,label=left: $\theta_1^{t+1}$, minimum size = 3pt, inner sep =0] (F) at (-0.63,-2.25){} ;

% \node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
% \node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

% \node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3.5,0){} ;
% \node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3.5/2,-0/2){} ;

% \node[fill, draw, circle,label=left: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3, 0.5){} ;
% \node[fill, draw, circle,label=below: $\theta_4^{t+2}$, minimum size = 3pt, inner sep =0] (L) at (-2,-0){} ;

% %Connect the updates
% \draw [line width=0.5pt, ->] (B)-- (F);
% \draw [line width=0.5pt, dashed] (F)-- (E);

% \draw [line width=0.5pt, ->] (A)-- (H);
% \draw [line width=0.5pt, dashed] (H)-- (G);

% \draw [line width=0.5pt, ->] (A)-- (J);
% \draw [line width=0.5pt, dashed] (J)-- (I);

% \draw [line width=0.5pt, ->] (B)-- (L);
% \draw [line width=0.5pt, dashed] (L)-- (K);

% \end{tikzpicture}
	
% 	\caption{Schematics illustrating the clients' similarities detection method when considering all the clients, left, and when sampling clients, right. $\theta^t$ is the global model at iteration $t$ and $\theta_i^{t+1}$ is the updated local model of client $i$ on $\theta^t$ while converging to its local optimum $\theta_i^*$.}
% 	\label{fig:schematic_sim}
% \end{figure}





\begin{figure}
\begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

%Global models
\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
\node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-7.5/4/2, -7.5/2/4){} ;

%Connect the globsl models
\draw [line width=1pt, ->] (A)-- (B);
%	\draw [line width=1pt, ->] (B)-- (C);
%	
%Local optima and local update
\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
\node[fill, draw, circle,label=below: $\theta_1^{t+1}$, minimum size = 3pt, inner sep =0] (F) at (-0.5/2,-2.7/2){} ;

\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;

\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
\node[fill, draw, circle,label=below: $\theta_4^{t+1}$, minimum size = 3pt, inner sep =0] (L) at (-3.5/2,-0.5/2){} ;

%Connect the updates
\draw [line width=0.5pt, ->] (A)-- (F);
\draw [line width=0.5pt, dashed] (F)-- (E);

\draw [line width=0.5pt, ->] (A)-- (H);
\draw [line width=0.5pt, dashed] (H)-- (G);

\draw [line width=0.5pt, ->] (A)-- (J);
\draw [line width=0.5pt, dashed] (J)-- (I);

\draw [line width=0.5pt, ->] (A)-- (L);
\draw [line width=0.5pt, dashed] (L)-- (K);


%\end{scriptsize}
\end{tikzpicture}
%	\hspace{1cm}
\begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

%Global models
\node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
\node[fill, draw, circle,label=right: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-2.5/2/2, -3/2/2){} ;
\node[fill, draw, circle,label=below: $\theta^{t+2}$, minimum size = 3pt, inner sep =0] (C) at (-1.9, -1.6){} ;

%Connect the globsl models
\draw [line width=1pt, ->] (A)-- (B);
\draw [line width=1pt, ->] (B)-- (C);
%	
%Local optima and local update
\node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-0.5,-2.7){} ;
\node[fill, draw, circle,label=below: $\theta_1^{t+2}$, minimum size = 3pt, inner sep =0] (F) at (-0.55,-1.7){} ;

\node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
\node[fill, draw, circle,label=right: $\theta_2^{t+1}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

\node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
\node[fill, draw, circle,label=above: $\theta_3^{t+1}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;

\node[fill, draw, circle,label=below: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -0.5){} ;
\node[fill, draw, circle,label=below: $\theta_4^{t+2}$, minimum size = 3pt, inner sep =0] (L) at (-2.25,-0.62){} ;

%Connect the updates
\draw [line width=0.5pt, ->] (B)-- (F);
\draw [line width=0.5pt, dashed] (F)-- (E);

\draw [line width=0.5pt, ->] (A)-- (H);
\draw [line width=0.5pt, dashed] (H)-- (G);

\draw [line width=0.5pt, ->] (A)-- (J);
\draw [line width=0.5pt, dashed] (J)-- (I);

\draw [line width=0.5pt, ->] (B)-- (L);
\draw [line width=0.5pt, dashed] (L)-- (K);

\end{tikzpicture}
	
	\caption{Schematics illustrating the clients' similarities detection method when considering all the clients, left, and when sampling clients, right. $\theta^t$ is the global model at iteration $t$ and $\theta_i^{t+1}$ is the updated local model of client $i$ on $\theta^t$ while converging to its local optimum $\theta_i^*$.}
	\label{fig:schematic_sim}
\end{figure}





% \begin{figure}
% \begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

% %Global models
% \node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
% \node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-7.5/4/2, -7.5/2/4){} ;

% %Connect the globsl models
% \draw [line width=1pt, ->] (A)-- (B);
% %	\draw [line width=1pt, ->] (B)-- (C);
% %	
% %Local optima and local update
% \node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-1.5,-3.5){} ;
% \node[fill, draw, circle,label=right: $\theta_1^t$, minimum size = 3pt, inner sep =0] (F) at (-1.5/2,-3.5/2){} ;

% \node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
% \node[fill, draw, circle,label=right: $\theta_2^t$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

% \node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
% \node[fill, draw, circle,label=above: $\theta_3^t$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;

% \node[fill, draw, circle,label=left: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -1){} ;
% \node[fill, draw, circle,label=below: $\theta_4^t$, minimum size = 3pt, inner sep =0] (L) at (-3.5/2,-1/2){} ;

% %Connect the updates
% \draw [line width=0.5pt, ->] (A)-- (F);
% \draw [line width=0.5pt, dashed] (F)-- (E);

% \draw [line width=0.5pt, ->] (A)-- (H);
% \draw [line width=0.5pt, dashed] (H)-- (G);

% \draw [line width=0.5pt, ->] (A)-- (J);
% \draw [line width=0.5pt, dashed] (J)-- (I);

% \draw [line width=0.5pt, ->] (A)-- (L);
% \draw [line width=0.5pt, dashed] (L)-- (K);


% %\end{scriptsize}
% \end{tikzpicture}
% %	\hspace{1cm}
% \begin{tikzpicture}[scale = 0.7, line cap=round,line join=round,>=triangle 45,x=1cm,y=1cm]

% %Global models
% \node[fill, draw, circle,label=above: $\theta^t$, minimum size = 3pt, inner sep =0] (A) at (0,0){} ;
% \node[fill, draw, circle,label=below: $\theta^{t+1}$, minimum size = 3pt, inner sep =0] (B) at (-2.5/2/2, -3/2/2){} ;
% \node[fill, draw, circle,label=below: $\theta^{t+2}$, minimum size = 3pt, inner sep =0] (C) at (-8.5/2/2, -7.5/2/2){} ;

% %Connect the globsl models
% \draw [line width=1pt, ->] (A)-- (B);
% \draw [line width=1pt, ->] (B)-- (C);
% %	
% %Local optima and local update
% \node[fill, draw, circle,label=left: $\theta_1^*$, minimum size = 3pt, inner sep =0] (E) at (-1.5,-3.5){} ;
% \node[fill, draw, circle,label=right: $\theta_1^{t+1}$, minimum size = 3pt, inner sep =0] (F) at (-1.5/2,-3.5/2){} ;

% \node[fill, draw, circle,label=left: $\theta_2^*$, minimum size = 3pt, inner sep =0] (G) at (0.5,-3){} ;
% \node[fill, draw, circle,label=right: $\theta_2^{t}$, minimum size = 3pt, inner sep =0] (H) at (0.5/2,-3/2){} ;

% \node[fill, draw, circle,label=left: $\theta_3^*$, minimum size = 3pt, inner sep =0] (I) at (-3,0){} ;
% \node[fill, draw, circle,label=above: $\theta_3^{t}$, minimum size = 3pt, inner sep =0] (J) at (-3/2,-0/2){} ;

% \node[fill, draw, circle,label=left: $\theta_4^*$, minimum size = 3pt, inner sep =0] (K) at (-3.5, -1){} ;
% \node[fill, draw, circle,label=below: $\theta_4^{t+1}$, minimum size = 3pt, inner sep =0] (L) at (-4.5/2,-3.5/2/2){} ;

% %Connect the updates
% \draw [line width=0.5pt, ->] (B)-- (F);
% \draw [line width=0.5pt, dashed] (F)-- (E);

% \draw [line width=0.5pt, ->] (A)-- (H);
% \draw [line width=0.5pt, dashed] (H)-- (G);

% \draw [line width=0.5pt, ->] (A)-- (J);
% \draw [line width=0.5pt, dashed] (J)-- (I);

% \draw [line width=0.5pt, ->] (B)-- (L);
% \draw [line width=0.5pt, dashed] (L)-- (K);

% \end{tikzpicture}
	
% 	\caption{Schematics illustrating the clients' similarities detection method when considering all the clients, left, and when sampling clients, right. $\theta^t$ is the global model at iteration $t$ and $\theta_i^{t+1}$ is the updated local model of client $i$ on $\theta^t$ while converging to its local optimum $\theta_i^*$.}
% 	\label{fig:schematic_sim}
% \end{figure}






